PLAYER*: Enhancing LLM-based Multi-Agent Communication and Interaction in Murder Mystery Games

We introduce WellPlay, a reasoning dataset for multi-agent conversational inference in Murder Mystery Games (MMGs). WellPlay comprises 1,482 inferential questions across 12 games, spanning objectives, reasoning, and relationship understanding, and establishes a systematic benchmark for evaluating agent reasoning abilities in complex social settings. Building on this foundation, we present PLAYER*, a novel framework for Large Language Model (LLM)-based agents in MMGs. MMGs pose unique challenges, including undefined state spaces, absent intermediate rewards, and the need for strategic reasoning through natural language. PLAYER* addresses these challenges with a sensor-based state representation and an information-driven strategy that optimises questioning and suspect pruning. Experiments show that PLAYER* outperforms existing methods in reasoning accuracy, efficiency, and agent-human interaction, advancing reasoning agents for complex social scenarios.

==> introduction_v1.tex <==
\section{Introduction}
Recent advancements in LLMs capable of generating human-like responses have boosted the development of LLM-based agents \citep{llm-2023-soni, furchat-2023-cherakara}. Building on this progress, a series of studies focusing on multi-agent communications have showcased the emergence of social interactions, including cooperation \citep{camel-li2023, diplomacy-2022fair}, trust \citep{werewolf-xu2023}, deception \citep{avalon-wang2023}, and information propagation \citep{generative-agent-park2023}. 
%Despite these advances, building agents for Murder Mystery Games (MMGs) that intentionally interact with humans in dynamic environments remains challenging. 
However, the study of multi-agent \textbf{complex social reasoning}—where agents must infer others’ beliefs, plans, and hidden goals in dynamic environments—remains significantly underexplored. One major bottleneck is the lack of large-scale, high-quality benchmarks capturing such intricate interactions. Furthermore, current evaluation methods either focus solely on the final win/loss outcome or rely heavily on manual evaluation, which significantly limits the scope of analysis due to the high cost \citep{werewolf-xu2023, avalon-wang2023, murdergame-wu2024}. For instance, \citet{murdergame-wu2024} were only able to manually design 56 inferential questions for 4 selected MMGs.



\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{game-flow-newstory.jpeg}
    \caption{The murder mystery game involves players taking on roles, questioning suspects, and using deduction to identify the killer, all while pursuing their character-specific objectives.
    }
    \label{fig:overview}
\end{figure}

To address this gap, we introduce \textbf{WellPlay}, a new dataset containing 1,482 inferential questions across 12 diverse Murder Mystery Games (MMGs). WellPlay categorises questions into three types—objective, reasoning, and relation—enabling a more comprehensive and scalable evaluation of agents' reasoning capabilities beyond binary outcomes.
As shown in Figure~\ref{fig:overview}, MMGs are strategic games that involve 4-12 players assuming character roles with specific scripts and objectives. Gameplay unfolds through language-based negotiation and tactical coordination over $n$ rounds, with players limited to $m$ questions per round. The ultimate goal is to uncover the truth collaboratively while advancing individual objectives. At the end of the game, players vote on the suspected killer and evaluate their objective completion.

MMGs are script-based games, and each script can only be played once. This sets them apart from traditional games like Go, which feature \textbf{fixed settings} and \textbf{well-defined action spaces} that support strategic search. They also differ from social deduction games such as Werewolves (with voting) and Avalon (with mission outcomes), where players receive \textbf{intermediate rewards} in each round. In contrast, MMGs offer neither a clearly defined search space nor intermediate feedback during decision-making.
To address these challenges, we first define a state space for each character, capturing their mental and situational attributes. These states are encoded using \emph{sensor-based representations} that can be updated via natural language prompting. This enables agents to explore the space through generative question-answering interactions (\textbf{what to ask}) in real time, framed as a planning problem \citep{DBLP:journals/ijrr/KaramanF11,DBLP:journals/ijrr/GammellBS20}. 
For the issue of intermediate reward in searching, we design an Information Gain (IG) based heuristic objective which aims to balance existing searching results and the expected reward for further questions. After each action, the agent evaluates whether the current information can update the character states and narrow down the range of suspects. Meanwhile, our method focuses on extracting highly suspicious characters, creating a question-target selection framework guided by IG (\textbf{who to ask}). Compared to previous work, this framework optimises the information collection path, significantly improving system efficiency.


%Furthermore, current evaluation methods either focus solely on the final win/loss outcome or rely heavily on manual evaluation, which significantly limits the scope of analysis due to the high-cost \citep{werewolf-xu2023, avalon-wang2023, murdergame-wu2024}. For instance, \citet{murdergame-wu2024} were only able to manually designed 56 inferential questions for 4 selected MMGs. To address the evaluation problem, we constructed a dataset, WellPlay, containing 1,482 inferential questions across 12 MMGs. These questions are categorised into three types: objective, reasoning, and relation. Including the win rate metric used in previous works, this provides a more diverse evaluation framework.
We also recruited human players to interact with the agent. The results revealed that previous agents often overfit to agent-vs-agent interaction environments, exhibiting verbose and repetitive dialogues that detracted from the player experience. By integrating our goal-oriented pruner, these issues were significantly mitigated, resulting in more human-like agent behaviour and greatly enhancing player satisfaction.

In summary, we have made the following contributions: 
(1) We construct \textbf{WellPlay}, a dataset containing 1,482 inferential questions across 12 diverse MMGs, providing a more robust and fine-grained evaluation framework for multi-agent complex social reasoning.
(2) We propose \textbf{\agentname}, a framework that models character states through detective sensors and selects questions using an IG-based reward, addressing the challenges of planning in continuous language space without intermediate feedback.
%(1)We propose \agentname, a framework using detective sensors to define and optimise the search in continuous language space.
%(2) We introduce an IG-based reward to address the lack of intermediate rewards, improving agent behaviour and efficiency.
%(3) We construct WellPlay, a dataset with 1,482 inferential questions across diverse categories, offering a more robust evaluation framework.
(3) We construct a human-agent interaction platform. By integrating a goal-oriented pruner, we significantly reduce verbosity and enhance the agent's interaction quality and player experience.
\footnote{Our code and dataset are available at 
% \url{https://anonymous.4open.science/r/PLAYER-074C}}. 
% https://github.com/alickzhu/PLAYER
\url{https://anonymous.4open.science/r/PLAYER-074C}, along with detailed MMG rules and procedures.}
